Selective Attention: Enhancing Transformer through Principled Context Control

The attention mechanism within the transformer architecture enables the model to weigh and combine tokens based on their relevance to the query. While self-attention has enjoyed major success, it notably treats all queries $q$ in the same way by applying the mapping $V^\top\text{softmax}(Kq)$, where $V,K$ are the value and key embeddings respectively. In this work, we argue that this uniform treatment hinders the ability to control contextual sparsity and relevance. As a solution, we introduce the $\textit{Selective Self-Attention}$ (SSA) layer that augments the softmax nonlinearity with a principled temperature scaling strategy. By controlling temperature, SSA adapts the contextual sparsity of the attention map to the query embedding and its position in the context window. Through theory and experiments, we demonstrate that this alleviates attention dilution, aids the optimization process, and enhances the model's ability to control softmax spikiness of individual queries. We also incorporate temperature scaling for value embeddings and show that it boosts the model's ability to suppress irrelevant/noisy tokens. Notably, SSA is a lightweight method which introduces less than 0.5% new parameters through a weight-sharing strategy and can be fine-tuned on existing LLMs. Extensive empirical evaluations demonstrate that SSA-equipped models achieve a noticeable and consistent accuracy improvement on language modeling benchmarks.

==> OLD_intro.tex <==
% \begin{abstract}
% Attention mechanism is the central component of the transformer architecture as it enables the model to create learnable weighted combinations of the tokens that are relevant to the query. While self-attention has enjoyed major success, it notably treats all queries $q$ in the same way by applying the mapping $V^\top \text{softmax}(Kq)$. In this work, we argue that this uniform treatment hinders the ability to control contextual sparsity and relevance. To this aim, we introduce the ``\emph{Selective Self-Attention}'' (SSA) layer which augments the softmax nonlinearity with a principled temperature-scaling strategy. SSA utilizes a query-temperature to adapt the contextual sparsity of the softmax map to the specific query and its position in the context window. Through theory and experiments, we demonstrate that this alleviates attention dilution, aids the optimization process, and enhances the model's ability to assign distinct sparsity levels across queries. To enhance relevance control, we also introduce a value-temperature and show that it boosts the model's ability to suppress irrelevant/noisy tokens. \red{Extensive empirical evaluations corroborate that SSA noticeably improves the language modeling performance: DISCUSS IMPROVEMENT HERE.}

% %Despite their success, traditional attention models often lack the ability to selectively prioritize more relevant segments of input data, which can lead to suboptimal performance in complex tasks. Our research introduces the Selective Self-Attention (SSA) model, an innovative approach that incorporates a temperature-based modulation mechanism into the attention framework to enhance selectivity and focus. By applying data-dependent temperatures to modify the softmax calculation of the attention scores, SSA allows for dynamic adjustment of focus across different parts of the input sequence. We present a detailed formulation of the SSA, including its theoretical foundations and algorithmic implementation. Theoretical analysis suggests that SSA can achieve higher expressiveness over traditional attention models, particularly in scenarios involving hierarchical data structures. We validate these theoretical claims with empirical experiments on several benchmark NLP tasks, where SSA demonstrates superior performance, particularly in tasks requiring deep contextual understanding and differentiation among tokens of varying relevance. 
% \end{abstract}
\section{Introduction}
In the field of machine learning, attention mechanisms have become pivotal, particularly within the realm of natural language processing (NLP). Since the advent of the transformer model, attention-based architectures have consistently delivered state-of-the-art performance on a variety of tasks. These mechanisms allow models to focus on different parts of the input sequence when performing tasks, enhancing their ability to capture contextual relationships in data. However, traditional attention mechanisms treat all parts of the input sequence equally, which can lead to inefficiencies, particularly in complex sequences.

This paper introduces a novel approach termed Selective Self-Attention (SSA), which enhances the standard attention mechanism by incorporating a temperature-based modulation method. This method allows the attention mechanism to vary its focus dynamically, assigning different levels of importance to different tokens based on a learned temperature function. Such an approach promises to enhance the model's ability to discern and prioritize relevant information in a sequence, thereby improving performance on tasks requiring deep contextual understanding.

The concept of temperature in attention mechanisms is not merely a fine-tuning parameter but a fundamental shift in how attention is computed. By adjusting the softmax temperature of each token individually, the SSA approach allows for a more nuanced and selective attention distribution. This selective focus is particularly beneficial in handling hierarchical and structured data where the relevance of tokens can vary significantly across the sequence.

In developing the SSA framework, we draw inspiration from both theoretical insights and empirical results. Theoretical considerations suggest that SSA can achieve a more expressive attention model compared to traditional methods. Empirically, we explore the application of SSA in various NLP tasks, demonstrating its ability to outperform existing models by a significant margin, particularly in complex scenarios involving nested or hierarchical data structures.

providing data-controlled relative-positional information to Attention

Specifically, we make the following contributions:
\begin{itemize}
\item parameter efficient, while developed for temp-scale, extensible to other attention models
\item Decoupling semantics from specificity, attention dilution, weight growth, theory
\item value selectivity, denoising viewpoint
\item empirical impact, ppl gain and speedup
\end{itemize}

\begin{figure}[t!]
\centering
%\hspace{-35pt}
\begin{subfigure}[b]{0.92\textwidth}
    \centering
	\begin{tikzpicture}
		\node at (0,0) []{\includegraphics[width=\textwidth]{SelectiveAttention/img/text_heat_border.pdf}};
\end{tikzpicture}
\vspace{-15pt}
% \caption{Varying budget with $\alpha=\frac{1}{20}$}
\vspace{-3pt}
\label{fig:text_heat}
\end{subfigure}
\caption{A quote from Steve Jobs where tokens are highlighted according to their temperatures learned by the Selective Attention layer. Darker color corresponds to lower temperatures.}
%and is associated with sparse and more selective context.}
\vspace{-0.5cm}
\end{figure}

==> positional_adjustment.tex <==
\section{Theoretical Study of Position Adjustment}

\subsection{The Need for Temperature Scaling from an Approximation Lens}

\noindent\textbf{Notation.} Consider an input sequence $\X=[\x_1,\ldots,\x_N]^\top\in\R^{N\times d}$, where $\x_t\in\R^d$ is the input token at time $t$. Let $\csf{n}{\cdot}$ denote the causally-masked softmax which sets the future input entries (with $i>n$) to $-\infty$ prior to softmax. The $n^{th}$ row of the causal attention map is given by $\s^{n}=\csf{n}{\X\W\x_n}$ where $\W$ represents the trainable weights of the attention head. Here, we merged the key and query weights $\W_K,\W_Q$ within the parameter $\W=\W_K\W_Q^\top$ to simplify subsequent notation.



\subsubsection{Proof of Theorem \ref{position thm}}
%The orthogonal assumption is only to simplify notation. More generally, we need 
\begin{proof} We first show the success direction. Set $\W$ such that $\bb^\top\W=0$ and $\ab^\top\W\ab=\ab^\top\W\bb=1$. Such $\W$ exists thanks to the linear independence of $\ab,\bb$. Now plugging this $\W$ into \eqref{imba risk}, for each position, regardless of whether $\x_n=\ab$ or $\x_n=\bb$, we obtain
\[ 
\X^\top\csf{n}{\tau_n\cdot \X\W\x_n}=\frac{n_ae^{\tau_n}}{n_ae^{\tau_n}+(n-n_a)}\ab+\frac{(n-n_a)e^{\tau_n}}{n_ae^{\tau_n}+(n-n_a)}\bb.
\] 
We wish to ensure
\[ 
\frac{n_ae^{\tau_n}}{n_ae^{\tau_n}+(n-n_a)}=\frac{1}{1+(n/n_a-1)e^{-\tau_n}}=\frac{1}{1+\kappa_ne^{-\tau_n}}=\alpha.
\] 
This in turn implies 
\[ 
\kappa_ne^{-\tau_n}=\frac{1-\alpha}{\alpha}\iff \tau_n=\log\kappa_n+\log\frac{\alpha}{1-\alpha}.
\]

Next, we discuss the failure case of flat temperature. To do so, we will lower bound the loss over the queries $\x_n=\bb$. Set $M=e^{(\bb-\ab)^\top\W\bb}$. Following same argument as above, for fixed temperature, $\W$ will output a non-adaptive composition of the form 
\[ 
\X^\top\csf{n}{\X\W\bb}=\frac{1}{1+M\kappa_n}\ab+\frac{M\kappa_n}{1+M\kappa_n}\bb.
\]
Thus, the loss function will be lower bounded by (accounting for the prediction error in $\ab,\bb$ terms and their orthogonality)
\[ 
\Lc(\W)\geq \min_{M>0}\sum_{n:\x_n=\bb} (0.5-\frac{1}{1+M\kappa_n})^2+(0.5-\frac{M\kappa_n}{1+M\kappa_n})^2=\min_{M>0}\sum_{n:\x_n=\bb} 2\cdot(0.5-\frac{1}{1+M\kappa_n})^2.
\] 
Now since $\kappa_n\geq 1$ over both second, at least $1/2$ of the queries are $\x_n=\bb$. Similarly, at least $4/5$ of the queries are $\x_n=\bb$ over the last quadrant. We will lower bound the loss over the two scenarios depending on $M\geq 1/3$ or not. 

First, suppose $M\geq 1/3$, in that case, using $\kappa_n\geq 4$ over the last quadrant, the loss is lower bounded by
% and over the last quadrant, at least $3/4$ of the queries are $\x_n=\bb$. 
\[ 
\Lc(\W)\geq \min_{M>0}\frac{1}{N}\sum_{n\geq 3N/4,\x_n=\bb}2\cdot(0.5-\frac{1}{1+M\kappa_n})^2\geq \frac{2}{5}(0.5-\frac{1}{1+4/3})^2> 0.002.
\] 
where we used the fact that there are $\geq \frac{N}{5}=\frac{N}{4}\cdot\frac{4}{5}$ queries with $\x_n=\bb$ over the last quadrant.

Similarly, suppose $M\leq1/3$, in that case, using $\kappa_n\leq 2$ over second quadrant, the loss is lower bounded by
% and over the last quadrant, at least $3/4$ of the queries are $\x_n=\bb$. 
\[ 
\Lc(\W)\geq \min_{M>0}\frac{1}{N}\sum_{N/2\geq n\geq N/4,\x_n=\bb}2\cdot(0.5-\frac{1}{1+M\kappa_n})^2\geq \frac{1}{4}(0.5-\frac{1}{1+2/3})^2= 0.0025.
\] 
where we used the fact that there are at least $N/8$ queries with $\x_n=\bb$ over the second quadrant. Combining these two cases, we found that, for any choice of $\W$, the loss is lower bounded by $0.002$.
\end{proof}

\subsection{Connecting Sparse Attention to Temperature Scaling}

To discuss sparsity and temperature, let us consider a fixed attention row $n$ and introduce:
\begin{itemize}
\item $\s(\tau)=\csf{n}{\tau\cdot\X\W\x_n}$, the scaled attention scores with inverse-temperature $\tau>0$.
\item $\bs(\kappa)=\csf{n}{\X\W\x_n,\kappa}$ denote the sparse attention scores where the top-$\kappa n$ entries are retained and the rest are set to $0$ where $0\leq \kappa\leq 1$.
\end{itemize}

The connection between sparsity and temperature scaling is clear. For instance, the top entry of $\s(\tau)$ will be decreasing in $\tau$ whereas the entropy of $\s(\tau)$ will be increasing. Here, we would like to establish how temperature scaling rule can be mapped to a sparsity rule. We will do this under a power-law relevance assumption on the attention scores. Here, we assume that the attention scores admit two values and the fraction of larger/relevant attention scores follow a power-law as context window grows.
\begin{assumption}[Power-law relevance] Consider the vector of raw attention scores $\ab=\X\W\x_n$. Each entry of $\ab$ is either $c$ or $c_+=c+\gamma$ for some $\gamma>0$. Additionally, $n^{-\pow}$ fraction of the entries are equal to $c_+$ for some $\pow>0$.
\end{assumption}
Above $c_+$ is the score attained by the salient tokens, $\gamma$ is the score advantage of salient tokens over rest of the tokens, and $\pow$ dictates the fraction of the salient tokens. To proceed, we have the following lemma which identifies condition under which TS and sparse-attention exhibit the same softmax temperature behavior.%Larger $\pow$ implies small fraction of salient tokens, necessitating a larger tempera
%Observe that if $\pow>1$, $\sum_{i=1}^n s_i$ converges as context length $n$ grows to infinity. This is the scenario where the distribution has heavy tail and $\s$ has finite-effective sparsity. On the other hand, if $\pow\leq 1$, the sum diverges and the tail probabilities have infinite mass. If we assume that $\W$ is norm-bounded, the latter becomes a more realistic assumption since, for norm-bounded $\W$, the ratio of the largest and smallest attention scores will be upper bounded by a constant, although this constant can be very large (namely $e^{C\cdot\tf{\W}}$). This is also a key cause of the attention dilution we are trying to address. 
\begin{lemma} For any choice of $\tau=1+\alpha\log n>0$ and corresponding sparsity $\kappa=\frac{n^{-\alpha\gamma}}{1-n^{-\pow}}+n^{-\pow}$, we have that $\tin{\s(\tau)}=\tin{\bs(\kappa)}$.
\end{lemma}
This reveals the clear connection between temperature scaling and sparsification rules. Simplifying the above, this lemma advocates that the sparsification rule should follow the power law decay of $\kappa\approx n^{-\alpha\gamma\wedge \pow}$. Consistent with this lemma, our experiments demonstrate that sparsification with power-law results in respectable performance.

%Specifically, when $\pow$ is large (salient entries decay fast), we need to set $\kappa= n^{-\alpha\gamma}$ which reveals the clear connection between to temperature scaling.

\begin{proof} We first compute the top entry of $\s(\tau)$ as follows 
\[ 
\frac{s_1^\tau}{\sum_{i=1}^ns_i^{\tau}}=\frac{e^{\gamma\tau}}{ n^{1-\pow}e^{\gamma\tau}+(n-n^{1-\pow})}=\frac{1}{n^{1-\pow}+n (1-n^{-\pow})e^{-\gamma\tau}}%\approx n^{-1}e^{\gamma\tau}\wedge n^{\pow-1}.
\] 
%Set $\kappa\gg n^{-\pow}$. 
We similarly compute the top sparse attention score as
\[ 
\frac{s_1}{\sum_{i=1}^{\kappa}s_i}=\frac{e^{\gamma}}{ n^{1-\pow}e^{\gamma}+(\kappa-n^{-\pow})n}= \frac{1}{n^{1-\pow}+(\kappa-n^{-\pow}) e^{-\gamma}n}.%\approx e^{\gamma-\log n}\wedge e^{-(1-\pow)\log n}.
\] 
Combining these, the top softmax probabilities are matched by setting 
\[ 
(\kappa-n^{-\pow}) e^{-\gamma}= (1-n^{-\pow})e^{-\gamma\tau}\iff \kappa=\frac{e^{-\gamma(\tau-1)}}{1-n^{-\pow}}+n^{-\pow}.
\] 
\end{proof}

==> star_graph_theory.tex <==
\subsection{Approximation Theoretic Benefits of Query Selective Attention}
To further formalize this, let us consider the following Star Graph topology.
\[
\Pb_\star=\begin{bmatrix}1/K&1/K&\dots &1/K\\0&1&\dots &0\\0&\vdots&\vdots&0\\0&\dots&0&1 \end{bmatrix}    
\]
This $\Pb_\star$ choices corresponds to the scenario where Node $1$ is connected to all nodes including itself and all other nodes are only self-connected. In light of Lemma \ref{vanilla lower bound}, Node 1 has low specificity whereas other nodes are highly specific. The following proposition establishes a variation of Lemma \ref{vanilla lower bound} in terms of softmax approximation.
\begin{lemma}\redp{Currently no proof} \red{Suppose embedding dimension is $d=2$, $K\geq 4$, and the embeddings $\{\eb_i\}_{i=1}^K$ are unit norm. No self-attention map can express $\Pb_\star$ even if the embeddings $\{\eb_i\}_{i=1}^K$ are optimized as well. Specifically, for some $\eps>0$ and for all $\W,\Eb$ choices, we have that $\|\Pb_\star-\sft{\Eb\W\Eb^\top}\|\geq \eps$.} In contrast, for any $\{\eb_i\}_{i=1}^K$, choosing $\W=\Iden_d$, $\tau(\eb_1)=0$ and $\tau(\eb_i)\rightarrow \infty$ for $i\geq 2$, query-selective attention precisely expresses $\Pb_\star$.
\end{lemma}
Observe that, in the above lemma, we choose a small embedding dimension. In general, this is necessary to establish expressivity separation: As discussed in the supplementary material, if $d\geq K$, we can show that standard self-attention can express any $\Pb_\star$ up to arbitrarily small error whenever $\Eb$ is not rank deficient. However, recalling Lemma \ref{vanilla lower bound}, the associated optimization for standard self-attention might still be more challenging.

\begin{comment}
\begin{proof} \redp{IN PROGRESS} Let us prove the first claim. Let $\W\in\R^{2\times 2}$ and $\qb=\W^\top \eb_1$. Suppose $\|\sft{\Eb\W\Eb^\top}-\Pb_\star\|\leq \eps'$ where $\eps'$ is arbitrarily small. Since first row of $\Pb_\star$ is all equal, for an arbitrarily small $\eps$ (corresponding to $\eps'$), this implies that $|(\eb_i-\eb_1)^\top\W^\top\eb_1|\leq \eps$ for all $i\geq 2$. To proceed, we will use other rows of $\Pb_\star$ to establish a contradiction. Set $\db_i=\eb_i-\eb_1$. For all $i\neq 1$, we require that 
\[ 
\db_{ij}=(\eb_i-\eb_j)^\top \W^\top\eb_j=(\db_i-\db_j)^\top\W^\top (\eb_1+\db_i).
\]
Observe that
\[ 
|\db_{ij}- (\db_i-\db_j)^\top\W^\top\db_i|\leq 2\eps.
\]
Let us decouple $\eb_i=\alpha_i\qb+\beta_i\qb^\perp$ where $\qb^\perp$ is the unit norm orthogonal direction to $\qb$. Set $\balpha_i=\alpha_i-\alpha_0$. We know that $|\balpha_i|\leq \eps/\tn{\qb}^2$. We also know that
\[ 
\qb=\W^\top\eb_1=\alpha_0\W^\top\qb+\beta_0\W^\top\qb^\perp\implies \W^\top\qb^\perp=\beta_0^{-1}(\Iden-\alpha_0\W^\top)\qb.
\]
Now define $\babeta=\beta_i/\beta_0$. We can write
\begin{align}
\W^\top\eb_i&=\alpha_i\W^\top\qb+\beta_i\W^\top\qb^\perp\\
&=(\alpha_i-\frac{\beta_i\alpha_0}{\beta_0})\W^\top\qb+\frac{\beta_i}{\beta_0}\qb\\
&=(\alpha_i-\babeta_i\alpha_0)\W^\top\qb+\babeta_i\qb\\
&=(\balpha_i+(1-\babeta_i)\alpha_0)\W^\top\qb+\babeta_i\qb.
\end{align}
We require that
\begin{align}
\eb_j^\top\W^\top\eb_i&=\alpha_j\babeta_i\tn{\qb}^2+\alpha_j(\alpha_i-\babeta_i\alpha_0)\qb^\top\W^\top\qb+\beta_j(\alpha_i-\babeta_i\alpha_0){\qb^\perp}^\top\W^\top\qb\\
&=\alpha_j\babeta_iA +\alpha_j(\alpha_i-\babeta_i\alpha_0)B+\babeta_j(\alpha_i-\babeta_i\alpha_0)C\\
&=\alpha_j\babeta_i(A-\alpha_0B) +\alpha_j\alpha_i B+\babeta_j(\alpha_i-\babeta_i\alpha_0)C\\
&=\alpha_j[\alpha_i B+\babeta_i(A-\alpha_0B)]+\babeta_j(\alpha_i-\babeta_i\alpha_0)C
\end{align}
\end{proof}
\end{comment}
%Are there stochastic matrices $\Pb_\star$, which can be represented by query-selective attention \emph{}


%Denote $[N]=\{1,\dots,N\}$ and $\Iden_d$ to be the identity matrix of size $d$. Let $\Pb\in\R^{N\times N}$ be a stochastic matrix whose rows add up to 1. Specifically, we assume that $\Pb$ is the transition matrix associated to a graph of $N$ nodes. Each node $i\in [N]$ can transition to its set of neighbors $\Nc(i)$ with equal probability. That means, the entries in the $i$'th row of $\Pb$ is equal to $1/\Nc(i)$ for entries corresponding to the neighbors and $0$ entries of non-neighbors.


%attention weights may have poor condition number or 
%finding large weights will be more challenging optimization , for instance, larger attention weights could
%the model can get away with small weights (even accounting for 
